Deep Learning on Real Geophysical Data: A Case Study for Distributed Acoustic Sensing Research

Deep Learning approaches for real, large, and complex scientific data sets can be very challenging to design. In this work, we present a complete search for a finely-tuned and efficiently scaled deep learning classifier to identify usable energy from seismic data acquired using Distributed Acoustic Sensing (DAS). While using only a subset of labeled images during training, we were able to identify suitable models that can be accurately generalized to unknown signal patterns. We show that by using 16 times more GPUs, we can increase the training speed by more than two orders of magnitude on a 50,000-image data set.

==> Makefile <==
###############################################################################
# the latex command is pdflatex
LATEX = pdflatex
# the bibtex command is biber -- specified in preamble.tex in this directory
BIBTEX = bibtex

###############################################################################
# the main latex file is iptf-ccgrid20.tex in this directory
MAIN = main

###############################################################################
# Assume all LaTeX files (*.tex) are in this level and all figures are in figs
# directory and all bibtex entries are at this level with .bib
TEXFILES = ${wildcard *.tex}
BIBFILES = ${wildcard *.bib}
FIGS = ${wildcard *.pdf}

###############################################################################
# default target
.DEFAULT_GOAL := $(MAIN).pdf
$(MAIN): $(MAIN).pdf
.PHONY: $(MAIN) clean realclean

###############################################################################
# run LATEX command to generate the main PDF file
$(MAIN).pdf $(MAIN).log: $(TEXFILES) $(FIGS) $(BIBFILES)
	${LATEX} $(MAIN)
	@if [ `fgrep undefined $(MAIN).log | fgrep Citation - | wc -l` -gt 0 ]; then \
	${BIBTEX} $(MAIN); ${LATEX} $(MAIN); fi;
	@if [ `fgrep undefined $(MAIN).log | fgrep Citation - | wc -l` -gt 0 ]; then \
	${BIBTEX} $(MAIN); ${LATEX} $(MAIN); fi;
	@while [ `fgrep -i 'Rerun ' $(MAIN).log | fgrep LaTeX - | wc -l` -gt 0 ]; do \
        ${LATEX} $(MAIN); \
        done

###############################################################################
# basic sanity check
check: missingincludes badrefs badbibs

# Extract a list of missing smartinclude files
missingincludes: $(MAIN).log
	@(grep -i "smartinclude: warning:" $< | \
	  sed 's/smartinclude: WARNING: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== SMARTINCLUDE WARNINGS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

# Check log for: 
# - Multiply defined labels
# - Undefined labels
# - Undefined citations
# - Undefined acronyms (no messages for multiply-defined acronyms)
badrefs: $(MAIN).log
	@(grep -i "latex warning:" $< |\
	  grep -v -i "there were multiply-defined labels" | \
	  grep "multiply defined" |\
	  sed 's/LaTeX Warning: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MULTIPLY-DEFINED LABELS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "latex warning:" $< | \
	  grep -v -i "there were undefined references" | \
	  grep -i "reference" | grep -i "undefined" |\
	  sed 's/LaTeX Warning: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED LABELS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "package acronym warning:" $< | \
	  grep -i "acronym" | grep -i "not defined" |\
	  sed 's/Package acronym Warning: //' |\
	  sort | uniq > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED ACRONYMS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

# Check BibTeX log for:
# - missing .bib files
# - missing database entries
# - repeated entries
# - string name undefined
# - errors in entries ("I was expecting...")
badbibs: $(MAIN).log
	${BIBTEX} $(MAIN)
	@(grep -i "i couldn't open database file " $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MISSING BIB FILES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "warning--i didn't find a database entry for" \
	  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MISSING BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "repeated entry--"  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== REPEATED BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "warning--string name" $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED STRINGS IN BIB =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "i was expecting"  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== ERRORS IN BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

clean:
	-@find . \( -name '*.aux' -print \) -o \( -name '*.log' -print \) \
		-o \( -name '*.bbl' -print \) -o \( -name '*.blg' -print \) \
		-o \( -name '*.toc' -print \) -o \( -name '*.out' -print \) \
		-o \( -name '*.bcf' -print \) -o \( -name '*~' -print \) \
		-o \( -name '*.maf' -print \) -o \( -name '*.mtc*' -print \) | xargs $(RM)

###############################################################################
# WARNING: removes the main target
realclean: clean
	$(RM) $(MAIN).pdf*

